Decentralized State Estimation via a Hybrid of Consensus and Covariance intersection

This paper presents a new recursive information consensus filter for decentralized dynamic-state estimation. No structure is assumed about the topology of the network and local estimators are assumed to have access only to local information. The network need not be connected at all times. Consensus over priors which might become correlated is performed through Covariance Intersection (CI) and consensus over new information is handled using weights based on a Metropolis Hastings Markov Chains. We establish bounds for estimation performance and show that our method produces unbiased conservative estimates that are better than CI. The performance of the proposed method is evaluated and compared with competing algorithms on an atmospheric dispersion problem.

==> TemplateFiles/inc.tex <==
\IEEEoverridecommandlockouts \overrideIEEEmargins 
%\pagestyle{plain}
\usepackage{TemplateFiles/fullpage}
\usepackage[ruled,vlined,linesnumbered]{TemplateFiles/algorithm2e}
\usepackage{mathrsfs}
\usepackage{graphicx}
\usepackage{amsfonts}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{array}
\usepackage{flafter}
%\usepackage{cite}
\usepackage{subfigure}
\usepackage{verbatim}
%\usepackage{bbm}
\usepackage[usenames]{color}
\usepackage[svgnames]{xcolor}
\usepackage{psfrag}
\usepackage{umoline}
\usepackage{hyperref}
%\usepackage{appendix} %[2009/09/02 v1.2b extra appendix facilities]
\let\proof\relax
\let\endproof\relax
\usepackage{amsthm}	% This is needed for \newtheorem and proof environment.
%\usepackage{natbib} % for citing the papers with auther-year format in parantheses.

\providecommand{\citet}[1]{\citeauthor{#1}\,[\citeyear{#1}]}
\providecommand{\citep}[1]{\cite{#1}}

\newtheorem{thm}{Theorem}
\newtheorem{Def}{Definition}
\newtheorem{Problem}{Problem}
\newtheorem{Lem}{Lemma}
\newtheorem{Cor}{Corollary}
\newtheorem{assumption}{Assumption}
\newtheorem{proposition}{Proposition}
\newtheorem{definition}{Definition}
\newtheorem{property}{Property}
\newtheorem{Remark}{Remark}
\newtheorem{exmp}{Example}[section]
%\newenvironment{proof}[1][Proof]{\begin{trivlist}
%\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newcommand{\TypeOfDoc}{IJRR} % This either can be TR or Conf or IJRR
\newcommand{\FinalFlag}{No} % This either can be No or Accepted

\graphicspath{{./figs/}}

\allowdisplaybreaks[1]

%\newcommand{\kXX}[1]{\color{blue} XX #1 XX \color{black}}
%\newcommand{\AXX}[1]{\color{orange} XX #1 XX \color{black}}
\newcommand{\aXX}[1]{\color{purple} #1 \color{black}}
